Dynamical Isometry and a Mean Field Theory of RNNs: Gating Enables Signal Propagation in Recurrent Neural Networks

Recurrent neural networks have gained widespread use in modeling sequence data across various domains. While many successful recurrent architectures employ a notion of gating, the exact mechanism that enables such remarkable performance is not well understood. We develop a theory for signal propagation in recurrent networks after random initialization using a combination of mean field theory and random matrix theory. To simplify our discussion, we introduce a new RNN cell with a simple gating mechanism that we call the minimalRNN and compare it with vanilla RNNs. Our theory allows us to define a maximum timescale over which RNNs can remember an input. We show that this theory predicts trainability for both recurrent architectures. We show that gated recurrent networks feature a much broader, more robust, trainable region than vanilla RNNs, which corroborates recent experimental findings. Finally, we develop a closed-form critical initialization scheme that achieves dynamical isometry in both vanilla RNNs and minimalRNNs. We show that this results in significantly improvement in training dynamics. Finally, we demonstrate that the minimalRNN achieves comparable performance to its more complex counterparts, such as LSTMs or GRUs, on a language modeling task.

==> backup_minimalrnn_init.tex <==
% !TEX root = icml2018_main.tex
In the previous subsection, we derived a quantity $\chi_1$ that defines the boundary between the ordered and the chaotic phases of forward propagation. Here we show that it also defines the boundary between exploding and vanishing gradients. To see this, consider the Jacobian of the state-to-state transition operator,
\begin{equation}
    \bm{J}_t  = \frac{\partial \bm{h}^{t+1}}{\partial \bm{h}^t} = \bm{D}_{\bm{u}^t} + \bm{D}_{\sigma'(\bm{v}^t)\odot(\bm{h}^{t-1}-\bm{z}^t)} \bm{W}\,,
\end{equation}
where $\bm{D}_{\bm{x}}$ is the diagonal matrix with $\bm{x}$ along its diagonal. We can compute the expected norm-squared of back-propagated error signals, which measures the growth or shrinkage of gradients. It is equal to the mean-squared singular value of the Jacobian~\cite{poole2016,schoenholz2016} or the first moment of $\bm{J}_t\bm{J}_t^T$,
\begin{equation}
\begin{split}
\frac{1}{N}\mathbb E[ \tr(\bm{J}_t\bm{J}_t^T)] = \mathbb E[ (u^t_1)^2] + \sigma_w^2 \mathbb E[\sigma'(v^t_1)^2(h^{t-1}_1-z_1^t)^2] \,,
\end{split}
\end{equation}
where we have used the fact that the elements of $\bm u^t$, $\bm h^t$ and $\bm z^t$ are i.i.d. Since we assume convergence to the fixed point, these distributions are independent of $t$ and it is easy to see that $\frac{1}{N}\mathbb E[\tr(\bm{J}_t\bm{J}_t^T)] = \chi_1$. The variance of back-propagated error signals through $T$ time steps is therefore $\frac{1}{N}\mathbb E[\tr({\bm J}{\bm J}^T)] = \chi_1^T$. As such, the constraint $\chi_1 = 1$ defines the boundary between phases of exponentially exploding and exponentially vanishing gradient variances. Note that unlike in the case of forward signal propagation, in the case of backpropagation this is independent of $\Sigma$.

As argued in~\cite{pennington2017resurrecting,PenningtonSG18}, controlling the variance of back-propagated gradients is necessary but not sufficient to guarantee trainability, especially for very deep networks. Beyond the first moment, the entire distribution of eigenvalues of ${\bm J}{\bm J}^T$ (or of singular values of ${\bm J}$) is relevant. Indeed, it was found in~\cite{pennington2017resurrecting,PenningtonSG18} that enabling dynamical isometry, namely the condition that all singular values of ${\bm J}$ are close to unity, can drastically improve training speed for very deep feed-forward networks.

Following~\cite{pennington2017resurrecting,PenningtonSG18}, we use tools from free probability theory to compute the variance $\sigma^2_{{\bm J}{\bm J}^T}$ of the limiting spectral density of ${\bm J}{\bm J}^T$; however, unlike previous work, in our case the relevant matrices are not symmetric and therefore we must invoke tools from non-Hermitian free probability, see~\cite{cakmak2012non} for a review. As in previous section, we make the simplifying assumption that the weights are untied, relying on the same motivations given in section~\ref{vanilla}. Using these tools, an un-illuminating calculation reveals that,
\begin{equation}
\label{eq:eigen_variance}
    \sigma^2_{{\bm J}{\bm J}^T} = \chi_1^{2T} \left(1 + T \frac{2(\mu_1-s_1) \mu_2+\sigma_1^2 + \sigma_2^2}{\chi_1^2} \right)\,,
\end{equation}
where,
\begin{eqnarray}
\label{eq:minimal_chi1}
%\begin{split}
\mu_1 &=& \int \mathcal{D}z\;\sigma^2(\sqrt{q^*} z + \mu_b) \\
\sigma_1^2 &=& -\mu_1^2 + \int \mathcal{D}z\; \sigma^4(\sqrt{q^*} z + \mu_b)\nonumber\\
\mu_2 &=& \sigma_{w}^2 (Q^* + R)\int \mathcal{D}z\;[\sigma'(\sqrt{q^*}z+\mu_b)]^2\nonumber\\
\sigma_2^2 &=& -\mu_2^2 + \sigma_{w}^4 ((Q^*)^2 + R^2)\int \mathcal{D}z\;[\sigma'(\sqrt{q^*}z+\mu_b)]^4\nonumber
%\end{split}
\end{eqnarray}
and $s_1$ is the first term in the Taylor expansion of the S-transform of the eigenvalue distribution of $WW^T$~\cite{PenningtonSG18}. For example, for Gaussian matrices, $s_1 = -1$ and for orthogonal matrices $s_1 = 0$.

Some remarks are in order about eq.~(\ref{eq:eigen_variance}). First, we note the duality between the forward and backward signal propagation (eq.~(\ref{eq:minimal_chi_c}) and eq.~(\ref{eq:minimal_chi1})).  For critical initializations, $\chi_1 = 1$, so $\sigma^2_{{\bm J}{\bm J}^T}$ does not grow exponentially, but it still grows linearly with $T$. This situation is entirely analogous to the feed-forward analysis of~\cite{pennington2017resurrecting,PenningtonSG18}. In the case of the vanilla RNN, the coefficient of the linear term is proportion to $q^*$, and can only be reduced by taking the weight and bias variances $(\sigma_w^2, \sigma_b^2) \to (1,0)$. A crucial difference in the minimalRNN is that the coefficient of the linear term can be made arbitrarily small by simply adjusting the bias mean $\mu_b$ to be positive, which will send $\mu_2 \to 0$ and $\mu_1 \to 1$ independent of $\Sigma$. Therefore the conditions for dynamical isometry decouple from the weight and bias variances, implying that trainability can occur for a higher-dimensional, more robust, slice of parameter space. Moreover, the value of $s_1$ has no effect on the capacity of the minimalRNN to achieve dynamical isometry. We believe these are fundamental reasons why gated cells such as the minimalRNN perform well in practice.

Algorithm~\ref{alg:crit_init} describes the procedure to find $\sigma_w^2, \sigma_v^2$ and $\sigma_b^2$ to achieve $\chi_1$ condition for minimalRNN. Given $\sigma_w^2, \sigma_v^2, \sigma_b^2$, we then construct the weight matrices and biases accordingly. $Q^\ast$ is used to initialize the $h^0$ to avoid transient phase. 


% \begin{algorithm}
% \caption{Critical initialization for minimalRNN}\label{alg:crit_init}
% \begin{algorithmic}[1]
% \Procedure{CriticalInit}{$q^\ast,\mu_b,R$}
% \State $EU \gets \int \mathcal{D}z\;\sigma(\sqrt{q^*} z + \mu_b)$
% \State $U^\ast \gets \int \mathcal{D}z\;\sigma^2(\sqrt{q^*} z + \mu_b)$
% \State $Q^\ast\gets R(1-2EU+U^\ast)/(1-U^\ast)$
% \State $\sigma_w^2 \gets (1-U^\ast) /(Q^\ast + R) / \int \mathcal{D}z\;[\sigma'(\sqrt{q^*}z+\mu_b)]^2$
% \State $\sigma_v^2 \gets (q^\ast - Q^\ast\sigma_w^2)/R$
% \State $\sigma_b^2 \gets 0$
% \State \textbf{return} $\sigma_w^2, \sigma_v^2, \sigma_b^2, Q^\ast$
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}[H]
\DontPrintSemicolon
%\SetAlgoLined
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\Input{$q^\ast,\mu_b,R$}
\Output{$\sigma_w^2, \sigma_v^2, \sigma_b^2, Q^\ast$}
\BlankLine
\hspace{6pt}$u \gets \int \mathcal{D}z\; \sigma(\sqrt{q^*} z + \mu_b)$\\
$\mu_1 \gets \int \mathcal{D}z\;\sigma^2(\sqrt{q^*} z + \mu_b)$\\
$Q^\ast\gets R(1-2u+\mu_1)/(1-\mu_1)$\\
$\sigma_w^2 \gets (1-\mu_1) /(Q^\ast + R) / \int \mathcal{D}z\;[\sigma'(\sqrt{q^*}z+\mu_b)]^2$\\
$\sigma_b^2 \gets 0$\\
$\sigma_v^2 \gets (q^\ast - Q^\ast\sigma_w^2 - \sigma_b^2)/R$
\caption{Critical initialization for minimalRNN}\label{alg:crit_init}
\end{algorithm}

==> backup_minimalrnn_meanfield.tex <==
% !TEX root = icml2018_main.tex

%Given a sequence of inputs $\bm x^t\in\mathbb R^M$, minimalRNN first maps its input $\bm x^t$ at each time step to a latent space through
%$$\bm{z}^t = \Phi(\bm{x}^t)$$
%$\Phi(\cdot)$ here can be any highly flexible functions such as a feed-forward network. In our experiment, we set $\Phi(\cdot)$ as a fully connected layer with $\tanh$ activation, that is, $\Phi(\bm{x}^t) = \tanh(\bm W_x\bm x^t$). 

To study the role of gating, we introduce the minimalRNN which is simpler than other gated RNN architectures but nonetheless features a gating mechanism. A sequence of inputs $\bm{x}^t\in\mathbb R^M$, is first mapped to the hidden space through
$\bm{z}^t = \Phi(\bm{x}^t)$\footnote{$\Phi(\cdot)$ here can be any highly flexible functions such as a feed-forward network. In our experiments, we take $\Phi(\cdot)$ to be a fully connected layer with $\tanh$ activation, that is, $\Phi(\bm{x}^t) = \tanh(\bm W_x\bm x^t)$.}. From here on, we refer to $\bm z^t \in \mathbb R^N$ as the inputs to minimalRNN.
The minimalRNN is then described by the recurrence relation,
\begin{eqnarray}\label{eq:minimal_rnn_h}
\bm{h}^t = \bm{u}^t \odot \bm{h}^{t-1} + (\bm{1}-\bm{u}^t) \odot \bm{z}^t 
\end{eqnarray}
where 
\begin{equation}\label{eq:minimal_rnn_f}
\bm{u}^t = \sigma(\bm{W} \bm{h}^{t-1} + \bm{V} \bm{z}^t + \bm{b})
\end{equation}
is the update gate. The minimalRNN retains the most essential gate in LSTMs~\cite{jozefowicz2015empirical,greff2017lstm} and achieves competitive performance. The simplified update of this cell enables us to pinpoint the role of gating in a more controlled setting. %In practice, we will frequently map the inputs $\bm x^t$ to a latent space before passing them to the minimalRNN.

As in the previous case we consider two sequences of inputs to the network, $\{\bm z_a^t\}$ and $\{\bm z_b^t\}$. We take $W_{ij}\sim\mathcal N(0, \sigma_w^2/N)$, $V_{ij}\sim\mathcal N(0, \sigma_v^2/N)$ and $b_i\sim\mathcal N(\mu_b,\sigma_b^2)$. We additionally define,
\begin{equation}
    \bm v_a^t = \bm W \bm h^{t-1}_a + \bm V\bm z^t_a + \bm b
\end{equation}
to be pre-activations to the gating function. By the central limit theorem (CLT) we can make a mean field assumption that $(v^t_{ia}, v^t_{jb})^T\sim\mathcal N(\mu_b,q^t_{ab}\delta_{ij})$ since $v^t_{ia}$ is a sum over $N$ i.i.d. random variables. Here,
\begin{equation}
q^t_{ab} = \sigma_w^2Q_{ab}^{t-1} + \sigma_v^2 R_{ab}^t + \sigma_b^2
\end{equation}
where we have defined $Q_{ab}^t = \mathbb E[h^t_{ia}h^t_{ib}]$ and $R_{ab}^t=\mathbb E[z^t_{ia}z^t_{ib}]$ to be the covariance between the hidden state and inputs respectively. We note that $R^t_{ab}$ is fixed by the input, but it remains for us to work out $Q^t_{ab}$. We find that (see SI section~\ref{supp:Q_recurrence}),
\begin{align}
Q_{ab}^t &\approx \mathbb E[u_{ia}^tu_{ib}^t]Q^{t-1}_{ab} + \mathbb E[(1-u_{ia}^t)(1-u_{ib}^t)]R^t_{ab} \label{eq:minimal_rnn_expectation}
\end{align}
where we assume that the expectation factorizes so that $h^{t-1}_{ia}$ and $u^t_{ia}$ are approximately independent. We believe this approximation becomes exact in the $N\to\infty$ limit.

We choose to normalize the data in a similar manner to the vanilla case so that $R_{aa}^t = R_{bb}^t = R$ independent of time. An immediate consequence of this normalization is that $Q_{aa}^t = Q_{bb}^t = Q^t$ and $q_{aa}^t = q_{bb}^t = q^t$. We then write $R_{ab}^t = R \Sigma^t$, $Q_{ab}^t = Q^tC^t$ and $q_{ab}^t = q^tc^t$ where $\Sigma^t$, $C^t$, and $c^t$ are cosine similarities between the inputs, the hidden states, and the pre-activations respectively. With this normalization, we can work out the mean-field recurrence relation characterizing the covariance matrix for the minimalRNN. This analysis can be done by either choosing a convention where we compute the recurrence relation for $\bm Q^t$ or $\bm q^t$. We will choose to study the dynamics of $\bm q^t$, however the two are trivially related. In SI section~\ref{supp:Q_fixed_point}, we analyze the dynamics of the diagonal term in the recurrence relation and prove that there is always a fixed point at some $q^*$. In SI section~\ref{supp:Q_dynamics}, we compute the depth scale over which $q^t$ approaches $q^*$. 

We now turn our attention to the dynamics of the cosine similarity between the pre-activations, $c^t$. As in the case of vanilla RNNs, we note that $q^t$ approaches $q^*$ quickly relative to the dynamics of $c^t$. We therefore choose to normalize the hidden state of the RNN so that $Q^0 = Q^*$ in which case both $Q^t=Q^*$ and $q^t=q^*$ independent of time. From eq.~\eqref{eq:minimal_rnn_expectation} it follows that the cosine similarity of the pre-activation evolves as,
%\begin{widetext}
\begin{align}\label{eq:minimal_rnn_off_diagonal_raw}
c^{t} &= (c^{t-1} + J_-\Sigma^{t-1}) \int D_{\bm q^{t-1}}\bm z\sigma(z_1)\sigma(z_2) \nonumber\\
&\hspace{2pc} - (J_+ + J_-)\Sigma^{t-1}\int D_{\bm q^{t-1}}\bm z\sigma(z_1) \nonumber\\
&\hspace{2pc} + \frac12[(J_+ + J_-)\Sigma^{t-1} + (J_+ - J_-)\Sigma^{t}]
\end{align}
%\end{widetext}
where we have defined $D_{\bm q}\bm z$ to be a gaussian measure in analogy to the vanilla case but with \emph{nonzero mean} $\mu_b$ and $J_{\pm} = (\sigma_w^2 \pm \sigma_v^2)R/q^*$.

As in the case of the vanilla RNN, we can study the behavior of $c^t$ in the vicinity of a fixed point, $c^*$. Similarly, by expanding eq.~\eqref{eq:minimal_rnn_off_diagonal_raw} to lowest order in $\epsilon^t = c^* - c^t$ we arrive at a linearized recurrence relation that has an exponential solution $\epsilon^{t+1} = \chi_{c^*}\epsilon^t$ where here,
\begin{align}\label{eq:minimal_chi_c}
    \chi_{c^*} &= \int D_{\bm q^*}\bm z\sigma(z_1)\sigma(z_2)\nonumber\\ &\hspace{2pc}+ q^*(c^* + J_-\Sigma)\int D_{\bm q^*}\bm z\sigma'(z_1)\sigma'(z_2).
\end{align}
The discussion above in the vanilla case carries over directly to the minimalRNN with the appropriate replacement of $\chi_{c^*}$. Unlike in the case of the vanilla RNN, here we see that $\chi_{c^*}$ itself depends on $\Sigma$. 

Again $c^* = 1$ is a fixed point of the dynamics only when $\Sigma = 1$. In this case, the minimalRNN experiences an order-to-chaos phase transition when $\chi_1 = 1$ at which point the maximum timescale over which signal can propagate goes to infinity. Similar to the vanilla RNN, when $\Sigma < 1$, we expect that the phase transition will be destroyed and the maximum duration of signal propagation will be severely limited. However, in a significant departure from the vanilla case, when $\mu_b\to\infty$ we notice that $\sigma(z + \mu_b) \to 1$, and $\sigma'(z + \mu_b)\to 0$ for all $z$. Considering eq.~\eqref{eq:minimal_chi_c} we notice that in this regime $\chi_{c^*}\to 1$ independent of $\Sigma$. In other words, gating allows for arbitrarily long term signal propagation in recurrent neural networks independent of $\Sigma$.

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{icml2018/figures/figure_1.pdf}
    \vspace{-0.2in}
    \caption{\textbf{Numerical verification of mean field results on the minimalRNN.} All experiments were done with fixed $\sigma_w = 6.88$, $\sigma_v = 1.39$, $R = 0.46$, and $\mu_b\in[-4,8]$. These hyperparameters are chosen so that the minimalRNN has an order-to-chaos critical point at $\mu_b = 0$. MC simulations were averaged over 1000 minimalRNNs with hidden dimension 8192. (a) Cosine similarity for theory (white dashed) compared with MC simulations of a minimalRNN with untied weights (solid). (b) Cosine similarity for tied weights (dashed) compared with untied weights (solid). (c) Comparison of $c^*$ for theory (white dashed), MC with untied weights (solid black), tied weights (dashed grey). (d) Comparison of linearized dynamics. Dashed lines show $A e^{-t/\tau}$ and solid lines show the result of simulations with untied weights. (e) Comparison of the timescale for signal propagation for different values of $\Sigma$.}
    \label{fig:mean_field_minimal}
\end{figure*}

We explore agreement between our theory and MC simulations of the minimalRNN in fig.~\ref{fig:mean_field_minimal}. In this set of experiments, we consider inputs such that $\Sigma^t = 0$ for $t < 10$ and $\Sigma^t = 1$ for $t\geq 10$. Fig.~\ref{fig:mean_field_minimal} (a,c,d) show excellent quantitative agreement between our theory and MC simulations. In fig.~\ref{fig:mean_field_minimal} (a,b) we compare the MC simulations of the minimalRNN with and without weight tying. While we observe that for many choices of hyperparameters the untied weight approximation is quite good (particularly when $c^*\approx 1$), deeper into the chaotic phase the quantitative agreement between breaks down. Nonetheless, we observe that the untied approximation describes the qualitative behavior of the real minimalRNN overall. In fig.~\ref{fig:mean_field_minimal} (e) we plot the timescale for signal propagation for $\Sigma = 1, 0.99,$ and $0$ for the minimalRNN with identical choices of hyperparameters. We see that while $\tau\to\infty$ as $\mu_b$ gets large independent of $\Sigma$, a critical point at $\mu_b = 0$ is only observed when $\Sigma = 1$. %\jp{Might be good to highlight the significance of this observation, like what does $\Sigma=1$ mean.}

%Unlike in the case of feed-forward networks, the nonlinear regime of eq.~\eqref{eq:minimal_rnn_off_diagonal_raw} can be long lived in the minimalRNN (see e.g. $\mu_b = 2$ in fig.~\ref{fig:mean_field_minimal} (d)). This is problematic, since signal propagation can become poor before the linearized dynamics described above becomes accurate. To account for this we consider the following ``nonlinear`` protocol for identifying a maximum depth of signal propagation. First, a threshold residual signal, $\epsilon^*$, is set that we take to be the smallest sensitivity of the outputs to the inputs that still allows the model to train. Then we identify $t^*$ such that $c^* - c^{t^*} = \epsilon^*$ and take it to be the maximum trainable depth of the minimalRNN. In cases where the transient is short lived and the linear approximation is valid and $t^* = \xi\log(A/\epsilon^*)$. That is, the linear depth scale identified above will set the value for $t^*$ up to a multiplicative factor (which was present in~\citet{schoenholz2016} as well). In cases where the transient is long lived and nonlinear effects will play a role we will typically see large deviations from the linear theory. In general the choice of $\epsilon^*$ is then \textit{the only free parameter} that we use to fit our theory with experiments. We plot these deviations in fig~\ref{fig:mean_field_minimal} (e). Strikingly, although the critical point is crucial in the linear theory, we observe that the transient dynamics are sufficient to affect signal propagation well before the linear regime becomes relevant. In general, as is shown in fig.~\ref{fig:depthscale} we observe that it is essential to take into account these nonlinear effects for the minimalRNN in making connection with trainability. 

==> backup_vanillarnn.tex <==

Vanilla RNNs are described by the recurrence relation,
\begin{equation}\label{eq:vanilla_rnn_recurrence}
    \bm h^t = \bm W\phi(\bm h^{t-1}) + \bm V \bm x^t + \bm b.
\end{equation}
Here $\bm x^t\in \mathbb R^M$ is the input, $\bm h^t\in\mathbb R^N$ is the pre-activation hidden state of the network and $\phi:\mathbb R\to\mathbb R$ is an arbitrary activation function. For the purposes of this discussion we will take $\phi=\tanh$. Furthermore, $\bm W\in\mathbb R^{N\times N}$ and $\bm V\in\mathbb R^{N\times M}$ are weight matrices that multiply the hidden state and inputs respectively and $\bm b\in\mathbb R^N$ is a bias.

%whose weights are randomly distributed, 
Next, we apply mean-field theory to vanilla RNNs following a similar strategy introduced in~\cite{poole2016,schoenholz2016}. At the level of mean-field theory, vanilla RNNs will prove to be intimately related to feed-forward networks and so this discussion proceeds analogously. For a more detailed discussion, see these earlier studies. 

%\textbf{Weight tying.} One peculiarity arises as there is no notion of weight tying in mean-field models. We will explore the ramifications of this approximation in making contact with experimental realizations of RNNs. Overall, we will see that while ignoring weight tying leads to quantitative differences between theory and experiment, it does not change the qualitative picture that emerges. See fig.~\ref{fig:mean_field_minimal} for verification of this in the case of the minimalRNN. \mc{update the figure????}

Consider two sequences of inputs $\{\bm x^t_1\}$ and $\{\bm x^t_2\}$, described by the empirical covariance matrix $R_{ab}^t = \frac1M\bm x^t_a\cdot\bm x^t_b$.  %such that $\bm x^t_a\in\mathbb R^M$. 
To simplify notation, we assume the input sequences have been standardized so that $R_{aa}^t = R_{bb}^t = R$ independent of time. %\footnote{All of the results in the paper can proceed without this assumption, but it introduces needless complication in the notation.}. 
This allows us to write $R_{ab}^t = R\Sigma^t$, where $\Sigma^t$ is the cosine similarity between the inputs at time $t$. 
These sequences are then passed into two identical copies of an RNN to produce two corresponding sequences of hidden states $\{\bm h^t_1\}$ and $\{\bm h^t_2\}$. As in~\citet{poole2016} we let the weights and biases be Gaussian distributed so that $W_{ij}\sim\mathcal N(0,\sigma_w^2/N)$, $V_{ij}\sim\mathcal N(0, \sigma_v^2/M)$, and $b_i\sim\mathcal N(0, \sigma_b^2)$, and we consider the wide network limit, $N\to\infty$. As in the fully-connected setting, we would like to invoke the Central Limit Theorem (CLT) to conclude that the hidden states are jointly Gaussian distributed. Unfortunately, in the recurrent setting, the CLT is violated due to the fact that $h^{t-1}_{ia}$ is correlated with $W_{jk}$ since weights are shared between steps of the RNN. 

To make progress, we proceed by developing the theory of signal propagation for RNNs with \emph{untied} weights. This allows for several simplifications, including the application of the CLT to conclude that  $(h^t_{ia},h^t_{jb})^T\sim\mathcal N(0,q^t_{ab}\delta_{ij})$, where $q_{ab}^t$ is independent of neuron index, $i$. We explore the ramifications of this approximation by comparing simulations of RNNs with tied and untied weights. Overall, we will see that while ignoring weight tying leads to quantitative differences between theory and experiment, it does not change the qualitative picture that emerges. See figs.~\ref{fig:mean_field_minimal} and~\ref{fig:depthscale} for verification.

%The use of the CLT here is therefore equivalant to approximating a recurrent neural network by a topologically identical model with untied weights.


With this approximation in mind, we will now quantify how the hidden states, $\{\bm h^t_a\}$, evolve. We convert the recurrence relation in eq.~\eqref{eq:mf_recurrence_vanilla_off_diag} over the $\bm h_a^t$ into a corresponding recurrence relation over the covariance matrix, $q^t_{ab}$. Using identical arguments to~\citet{poole2016} one can show that,
\begin{align}
    q^{t}_{aa} &= \sigma_w^2\int D_{\bm q^{t-1}}\bm z\phi(z_a)^2 + \sigma_v^2R + \sigma_b^2\label{eq:mf_recurrence_vanilla_diag}\\
    q^{t}_{ab} &= \sigma_w^2\int D_{\bm q^{t-1}}\bm z\phi(z_a)\phi(z_b) + \sigma_v^2R\Sigma^t + \sigma_b^2\label{eq:mf_recurrence_vanilla_off_diag}
\end{align}
%\jp{Do we want to allow $a=b$? Then we could have a single equation}
%\mc{Should we keep the recursion from $t-1$ to $t$ to be consistent with eq.(1)}
where $D_{\bm q}\bm z = dz_1dz_2 e^{-\frac12 z^T\bm q^{-1} z}/\sqrt{2\pi|\bm q|}$ is a Gaussian measure with covariance matrix $q_{ab}$. By symmetry, our normalization allows us to define $q_{aa}^t = q_{bb}^t = q^t$ to be the magnitude of the hidden state and $c^t = q_{ab}^t/q^t$ to be the cosine similarity between the hidden states. We will be particularly concerned with understanding the dynamics of the cosine similarity, $c^t$.

% $c^0$ is a free parameter and
In feed-forward networks, the inputs dictate the initial value of the cosine similarity, $c^0$ and then the evolution of $c^t$ is determined solely by the network architecture. By contrast in recurrent networks, inputs perturb $c^t$ at each timestep. Analyzing the dynamics of $c^t$ for arbitrary $\Sigma^t$ is therefore challenging, however significant insight can be gained by studying eq.~\eqref{eq:mf_recurrence_vanilla_off_diag} for $\Sigma^t = \Sigma$ independent of time. In the case of time-independent $\Sigma^t$, as $t\to\infty$ both $q^t\to q^*$ and $c^t\to c^*$ where $q^*$ and $c^*$ are fixed points of the variance of the hidden state and the cosine-similarity between hidden states respectively. As was discussed previously~\cite{poole2016,schoenholz2016}, the dynamics of $q^t$ are generally uninteresting provided $q^*$ is finite. We therefore choose to normalize the hidden state such that $q^0 = q^*$ which implies that $q^t = q^*$ independent of time.  

In this setting it was shown in~\citet{schoenholz2016} that in the vicinity of a fixed point, the term in eq.~\eqref{eq:mf_recurrence_vanilla_off_diag} can be expanded to lowest order in $\epsilon^t = c^* - c^t$ to give the linearized dynamics, $\epsilon^{t} = \chi_{c^*}\epsilon^{t-1}$ where
\begin{equation}\label{eq:chi_cstar_vanilla}
    \chi_{c^*} = \sigma_w^2\int D_{\bm q^*}\bm z\phi'(z_1)\phi'(z_2).
\end{equation}
These dynamics have the solution $\epsilon^t = \chi_{c^*}^{t-t_0}\epsilon^{t_0}$ where $t_0$ is the time when $c^t$ is close enough to $c^*$ for the linear approximation to be valid. If $\chi_{c^*} < 1$ it follows that $c^t$ approaches $c^*$ exponentially quickly over a timescale $\tau = -1/\log\chi_{c^*}$ and $c^*$ is called a stable fixed point. When $c^t$ gets too close to $c^*$ to be distinguished from it to within numerical precision, information about the initial inputs has been lost. Thus, $\tau$ sets the maximum timescale over which we expect the RNN to be able to remember information. If $\chi_{c^*} > 1$ then $c^t$ gets exponentially farther from $c^*$ over time and $c^*$ is an unstable fixed point. In this case, for the activation function considered here, another fixed point that is stable will emerge. Note that $\chi_{c^*}$ is independent of $\Sigma$ and so the dynamics of $c^t$ near $c^*$ do not depend on $\Sigma$. 

In vanilla fully-connected networks $c^* = 1$ is always a fixed point of $c^t$, but it is not always stable. Indeed, it was shown that these networks exhibit a phase transition where $c^* = 1$ goes from being a stable fixed point to an unstable fixed point as a function of the network's hyperparameters. This is known as the order-to-chaos transition and it occurs exactly when $\chi_1 = 1$. Since $\tau = -1/\log(\chi_1)$,  signal can propagate infinitely far at boundary between order and chaos.  Comparing eq.~\eqref{eq:mf_recurrence_vanilla_diag} and ~\eqref{eq:mf_recurrence_vanilla_off_diag}, 
we see that in recurrent networks, $c^* = 1$ is a fixed point only when $\Sigma = 1$, and in this case the discussion is identical to the feed-forward setting. When $\Sigma < 1$, it is easy to see that $c^* < 1$ since if $c^t = 1$ at some time $t$ then $c^{t+1} = 1 - \sigma_v^2R(1-\Sigma)/q^* < 1$. We see that in recurrent networks noise from the inputs destroys the ordered phase and there is no ordered-to-chaos critical point. As a result we should expect the maximum timescale over which memory may be stored in vanilla RNNs to be fundamentally limited by noise from the inputs. %In particular, we see that from eq.~\eqref{eq:mf_recurrence_vanilla_off_diag} if $c^0 = 1$ then $c^1 = 1 - \sigma_v^2R/q^*(1-\Sigma)$ and so the degree to which $c^* = 1$ is not a fixed point depends on the magnitude of $\sigma_v^2R/q^*$.

The end-to-end Jacobian  of a vanilla RNN with untied weights is in fact formally identical to the input-output Jacobian of a feedforward network, and thus the results from~\cite{pennington2017resurrecting} regarding conditions for dynamical isometry apply directly. In particular, dynamical isometry is achieved with orthogonal state-to-state transition matrices $\bm W$, $\tanh$ non-linearities, and small values of $q^*$. %It is logically possible that the untied weights assumption works well from the mean-field perspective, but breaks down when discussing dynamical isometry. Perhaps surprisingly, this is not the case. 
Perhaps surprisingly, these conclusions continue to be valid if the assumption of untied weights is relaxed. To understand why this is the case, consider the example of a linear network. For untied weights, the end-to-end Jacobian is given by $\hat{\bm J} = \prod_{t=1}^T \bm W_t$, while for tied weights the Jacobian is given by ${\bm J} = {\bm W}^T$. It turns out that as $N\to\infty$ there is sufficient self-averaging to overcome the dependencies induced by weight tying and the asymptotic singular value distributions of $\hat{\bm J}$ and $\bm J$ are actually identical \cite{haagerup2000brown}.

%To do this we will apply the random matrix theory approach presented in~\citet{pennington2017resurrecting} to compute the singular value distribution of the Jacobian of a vanilla RNN. As in the case of mean field theory, the spectrum of the Jacobian of vanilla recurrent networks is almost identical to that of fully-connected feed-forward networks.   

%\sss{DYNAMICAL ISOMETRY STUFF HERE!}

==> minimalrnn.tex <==
% !TEX root = icml2018_main.tex
%\jp{Should we move this relocate this subsection outside of the ``Theory'' section? Defining the architecture seems like it's of higher-level importance than a subsection in the theory section.}

%Gated RNNs such as LSTMs were first introduced as a mechanism to combat gradient exploding or vanishing in RNNs. Although it is intuitive to reason about how the gate units could modulate signal propagation, the complexity of these networks prevents us from fully understanding the machinery leading to better trainability. We therefore introduce a new variant of gated RNNs featuring a single gate, named minimalRNN. 


%Given a sequence of inputs $\bm x^t\in\mathbb R^M$, minimalRNN first maps its input $\bm x^t$ at each time step to a latent space through
$$\bm{z}^t = \Phi(\bm{x}^t)$$
$\Phi(\cdot)$ here can be any highly flexible functions such as a feed-forward network. In our experiment, we set $\Phi(\cdot)$ as a fully connected layer with $\tanh$ activation, that is, $\Phi(\bm{x}^t) = \tanh(\bm W_x\bm x^t$). Given this latent representation $\bm{z}^t$ of the input, minimalRNN then updates its states as,
\begin{eqnarray}\label{eq:minimal_rnn_h}
\bm{h}^t = \bm{u}^t \odot \bm{h}^{t-1} + (\bm{1}-\bm{u}^t) \odot \bm{z}^t 
\end{eqnarray}
where 
\begin{equation}\label{eq:minimal_rnn_f}
\bm{u}^t = \sigma(\bm{W} \bm{h}^{t-1} + \bm{V} \bm{z}^t + \bm{b})
\end{equation}
is the update gate. minimalRNN retains the most essential gate in LSTMs~\cite{jozefowicz2015empirical,greff2017lstm} and achieves competitive performance. The simplified update of this cell on the other hand, enables us to pinpoint the role of gating in a more controlled setting. 

%\textbf{Latent representation.} The dynamic of minimalRNN prescribed by these updates is fairly straight-forward. First, the encoder  $\Phi(\cdot)$ defines the latent space. The recurrent part of the model is then confined to move within this latent space.  At each step $t$, minimalRNN takes its previous state $\mathbf{h}_{t-1}$ and the encoded input $\mathbf{z}_t$, then simply outputs a weighted average of both depending on the gate $\mathbf{u}_t$.  That is,  dimension $i$ of the RNN state $h_t^i$  is activated by input $z^i_t$ and relax toward zero without any new input from988i that dimension. The rate of relaxation is determined by the gate $u_t^i$. It gets reactivated once it sees $z^i_t$ again. 


% Comparing with LSTM, GRU, minimalRNN resorts to a much simpler update inside the recurrent neural network.  The update rule bears some similarity to a recent work on Chaos Free recurrent neural networks~\cite{laurent2017chaos}, in that both forbid the mixing between different dimensions of the state. Only a single gate is used in minimalRNN comparing with two in GRUs and three in LSTMs. 

%retains the gating mechanism, which is known to be critical to preserve long range dependencies in RNNs. However, only one gate remains. The update rule bears some similarity to that of CFN, in that both forbid the mixing between different dimensions of the state. %The recurrent part of the model can be seen as a special case of the highway networks~\cite{srivastava2015training}. %In other words, each dimension of the  state $h^i_t$ is only influenced by the same dimension from previous state $h_{t-1}^i$, but not the other dimensions $h_{t-1}^j, j \neq i$.

%\begin{figure}
%%\hspace{0.1in}
%%\vspace{-0.1in}
% \begin{center}
%    \includegraphics[width=0.4\textwidth]{figures/minimalRNN.png}
% \end{center}
% \caption{Model architecture of minimalRNN.}
% \label{fig:mrnn}
%\end{figure}
%\mc{Not sure how much info the picture is adding, should leave it out if we are short on space.}
